RoboAgentLab: A Taxonomy and Open Research Platform for Agentic Robotics Across Acting, Building, and Evolving

Foundation models are extending the scope of robotic intelligence beyond task execution to the development and improvement of robot code and capabilities. This emerging paradigm, termed agentic robotics, where coding agents write and refine code for robots, calls for a unified account of what agents decide and how their decisions affect robot performance. We introduce a taxonomy organized around three complementary roles: Agent as Actor, which directs robot behavior; Agent as Infrastructure, which constructs resources and directs development workflows; and Agent as Evolver, which revises and retains system changes through feedback. We synthesize the design trade-offs across these roles by examining observation access, action authority, and what execution can reuse. Moving model computation into development changes the balance between online adaptation and preparation cost, while the value of retained programs, memories, and components depends on how they affect later runs. We introduce RoboAgentLab, an open research platform that records robot execution, memory reuse, and feedback-informed software revision. We identify future directions in efficient agentic decision-making, reliable evaluation of retained improvements, and training agents to continue robotics research.

==> figures/author-institutions.tex <==
\begingroup
\newsavebox{\institutionlogobox}
% ---- 统一的 logo 外框：每个 logo 在 \logoW × \logoH 内等比放到最大 ----
\newlength{\logoW}\setlength{\logoW}{20mm}   % 最大宽度
\newlength{\logoH}\setlength{\logoH}{7mm}    % 最大高度
\newcommand{\instlogo}[2][]{%
  \includegraphics[#1,width=\logoW,height=\logoH,keepaspectratio]{#2}}
\newcommand{\numberedinstitution}[2]{%
  \sbox{\institutionlogobox}{#2}%
  \makebox[\wd\institutionlogobox][l]{%
    \rlap{\raisebox{\dimexpr0.5\logoH+1.5mm\relax}[8.0mm][0pt]{\normalfont\fontsize{6.5}{7}\selectfont #1}}%
    \raisebox{-0.5\ht\institutionlogobox}{\usebox{\institutionlogobox}}}%
}
\noindent\makebox[\textwidth][c]{\hbox to \textwidth{%
\numberedinstitution{1}{\instlogo[trim={124.984bp 146.982bp 124.984bp 146.982bp},clip]{figures/institutions/nus.png}}\hfil%
\numberedinstitution{2}{\instlogo{figures/institutions/ntu.png}}\hfil%
\numberedinstitution{3}{\instlogo[trim={610bp 998bp 1314bp 436bp},clip]{figures/institutions/stanford-red-combinations.png}}\hfil%
\numberedinstitution{4}{\instlogo[trim={0bp 0bp 4.999bp 0bp},clip]{figures/institutions/berkeley.png}}\hfil%
\numberedinstitution{5}{\instlogo{figures/institutions/cmu-wordmark-red.png}}\hfil%
\numberedinstitution{6}{\instlogo[trim={276.014bp 410.021bp 276.014bp 410.021bp},clip]{figures/institutions/nvidia.png}}\hfil%
\numberedinstitution{7}{\instlogo[trim={0bp 1.5bp 1.5bp 0bp},clip]{figures/institutions/utexas.png}}%
}}\par\vspace{1mm}
\noindent\makebox[\textwidth][c]{\hbox to \textwidth{%
\numberedinstitution{8}{\instlogo[trim={14.998bp 13.998bp 14.998bp 13.998bp},clip]{figures/institutions/harvard.png}}\hfil%
\numberedinstitution{9}{\instlogo{figures/institutions/princeton.pdf}}\hfil%
\numberedinstitution{10}{\instlogo[trim={1bp 2bp 1bp 2bp},clip]{figures/institutions/oxford.png}}\hfil%
\numberedinstitution{11}{\instlogo[trim={23bp 20bp 23bp 20bp},clip]{figures/institutions/gatech.png}}\hfil%
\numberedinstitution{12}{\instlogo[trim={3.360bp 5.520bp 5.760bp 5.280bp},clip]{figures/institutions/astar.png}}\hfil%
\numberedinstitution{13}{\instlogo[trim={0bp 619bp 0bp 620bp},clip]{figures/institutions/mit-red-lockup.png}}\hfil%
\numberedinstitution{14}{\instlogo{figures/institutions/unc.pdf}}\hfil%
\numberedinstitution{15}{\instlogo[trim={125bp 180bp 130bp 145bp},clip]{figures/institutions/eaic.png}}%
}}\par
\endgroup 

==> figures/project-links.tex <==
\begingroup
\small\sffamily
\definecolor{resourcelinkbg}{HTML}{EFF5F8}
\definecolor{resourcelinkborder}{HTML}{CCDCE6}
\setlength{\fboxsep}{6pt}%
\setlength{\fboxrule}{0.4pt}%
\newcommand{\resourcelink}[3]{\href{#1}{\raisebox{-0.15em}{\includegraphics[height=1em]{figures/icons/#2.pdf}}\,\textbf{#3}}}%
\noindent\fcolorbox{resourcelinkborder}{resourcelinkbg}{%
\makebox[\dimexpr\textwidth-2\fboxsep-2\fboxrule\relax][c]{%
\resourcelink{https://roboagentlab.github.io/}{globe}{Website}\quad
\resourcelink{https://roboagentlab.github.io/docs/quickstart.html}{book-open}{Documentation}\quad
\resourcelink{https://github.com/RoboAgentLab/RoboAgentLab}{github}{Code}\quad
\resourcelink{https://github.com/RoboAgentLab/awesome-agentic-robotics}{github}{Awesome list}\quad
\resourcelink{https://huggingface.co/RoboAgentLab/datasets}{huggingface}{Datasets}}}\par
\endgroup

